Analysis of d-ary Tree Algorithms with Successive Interference Cancellation

In this article, we calculate the mean throughput, number of collisions, successes, and idle slots for random tree algorithms with successive interference cancellation. Except for the case of the throughput for the binary tree, all the results are new. We furthermore disprove the claim that only the binary tree maximises throughput. Our method works with many observables and can be used as a blueprint for further analysis.

==> Evaluation.tex <==
\section{Evaluation}
\label{sec:evaluation}

Main Responsibility is Quirin. \yd{This is just a filler section for now. I think this will be a sort of section explaining a bit more the results form the analysis. Some plots, delay analysis, collision analysis etc. }

==> Tables/STA_Table.tex <==
\renewcommand{\arraystretch}{1}
\setlength\tabcolsep{1pt}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
    \hline
      \multirow{2}{*}{\textbf{slot no.}} & \multicolumn{4}{c| } {\textbf{state of counter} } & {\textbf{feedback}} & {\textbf{feedback}}  \\ \cline {2-5}
        & \textbf{\textit{user1}} & \textbf{\textit{user2}} & \textbf{\textit{user3}} & \textbf{\textit{user4}} & \textbf{STA} & \textbf{SICTA} \\ \hline
      1         & 0     & 0     & 0     & 0   & e & e  \\ \hline
      2         & 0     & 1     & 0     & 0   & e & e  \\ \hline
      3         & 2     & 3     & 2     & 2   & 0 & 0  \\ \hline
      4         & 1     & 2     & 1     & 1   & 0 & 0  \\ \hline
      \rowcolor{Gray}
      5         & 0     & 1     & 0     & 0   & e & e  \\ \hline
      6         & 2     & 3     & 0     & 1   & 1 & 1  \\ \hline
      7         & 1     & 2     & x     & 0   & 1 & 3  \\ \hline
      \rowcolor{Gray}
      8         & 0     & 1     & x     & x   & 1 & x  \\ \hline
      \rowcolor{Gray}
      9         & x     & 0     & x     & x   & 1 & x  \\ \hline
      \rowcolor{Gray}
      10        & x     & x     & x     & x   & 0 & x  \\ \hline
    \end{tabular}
